Enhancing Retrieval Systems with Inference-Time Logical Reasoning

Traditional retrieval methods rely on transforming user queries into vector representations and retrieving documents based on cosine similarity within an embedding space. While efficient and scalable, this approach often fails to handle complex queries involving logical constructs such as negations, conjunctions, and disjunctions. In this paper, we propose a novel inference-time logical reasoning framework that explicitly incorporates logical reasoning into the retrieval process. Our method extracts logical reasoning structures from natural language queries and then composes the individual cosine similarity scores to formulate the final document scores. This approach enables the retrieval process to handle complex logical reasoning without compromising computational efficiency. Our results on both synthetic and real-world benchmarks demonstrate that the proposed method consistently outperforms traditional retrieval methods across different models and datasets, significantly improving retrieval performance for complex queries.

==> tables/more_terms.tex <==
\begin{table}
\setlength\tabcolsep{4pt}
\begin{tabular}{lrrrr}
\toprule
\textbf{N} & \textbf{base} & \textbf{uncalibrated} & \textbf{calibrated} & \textbf{random} \\
\midrule
\multicolumn{5}{l}{\textit{AND}:} \vspace{5pt}\\
10 & 0.49 & 0.53 & \textbf{0.57} & 0.44 \\
\multicolumn{5}{l}{\textit{OR}:} \vspace{5pt}\\
10 & 0.95 & 0.95 & \textbf{1.00} & 0.79 \\
\bottomrule
\end{tabular}
\caption{Scaling the number of terms. \felix{TODO: add number of positives/negatives in the data}}
\end{table}
